Average Elliptic Billiard Invariants with Spatial Integrals

We compare invariants of N-periodic trajectories in the elliptic billiard, classic and new, to their aperiodic counterparts via a spatial integrals evaluated over the boundary of the elliptic billiard. The integrand is weighed by a universal measure equal to the density of rays hitting a given boundary point. We find that aperiodic averages are smooth and monotonic on caustic eccentricity, and perfectly match N-periodic average invariants at the discrete caustic parameters which admit a given N-periodic family.

==> 070_ratio_of_areas.tex <==
\textcolor{red}{eliminate this section?}
The ratio of the area of the triangles $P_1P_2P_{12}'$ and  $0P_1P_2$
is given by

\[\frac{ a^2 x_0^2}{  a_0^4} +\frac{ b^2y_0^2 }{ b_0^4} - 1\]

Therefore the ratio of the areas of the quadrilateral (positively oriented) $P_1P_{12}'P_2 0$ and the triangle  $0P_1P_2$ is given by

\[\frac{ a^2 x_0^2}{  a_0^4} +\frac{ b^2y_0^2 }{ b_0^4}  \]

==> _not_used/075_invariant_table.tex <==
A list of $N$-periodic trajectory invariants appeared in \cite{reznik19,reznik2020-invariants} and are shown in Table~\ref{tab:invariants}. 

\begin{table}
\begin{tabular}{c|l|c|l|l|c}
symbol & invariant & value & which N & date & proven \\
\hline
$k_1$ & $\sum{\cos\theta_i}$ & $JL-N$ & all & 4/19 & \cite{akopyan2020-invariants,bialy2020-invariants} \\
$k_2$ & $\prod{\cos\theta'_i}$ & ? & all & 5/19 & \cite{akopyan2020-invariants,bialy2020-invariants} \\
$k_3$ & $A'/A$ & ? & odd & 8/19 & \cite{akopyan2020-invariants} \\
$k_4$ & $\sum{\cos(2\theta'_i)}$ & ? & all & 1/20 & \cite[Thm 6]{akopyan2020-invariants} \\
$k_5$ & $\prod{\sin(\theta_i/2)}$ & ? & odd & 1/20 & \cite[Thm 6]{akopyan2020-invariants} \\
$k_6$ & $A'A$ & ? & even & 1/20 & ? \\
$k_7$ & $k_3 k_5$ & ? & $N\,{\equiv}\,0 \Mod{4}$ & 1/20 & ? \\
$k_8$ & $k_3 / k_5$ & ? & $N\,{\equiv}\,2 \Mod{4}$ & 1/20 & ? \\
\end{tabular}
\caption{$N$-periodic invariants. $\theta_i$, $A$ (resp.~$\theta_i'$,$A'$) are angles,area of an N-periodic (resp.~tangent polygon to the N-periodic). $J=\left<Ax,v\right>$ (resp.~$L$) is Joachimsthal's (resp.~perimeter) invariants \cite{sergei91}. All sums/products go from $i=1$ to $N$.}
\label{tab:invariants}
\end{table}

==> _not_used/overflow.tex <==

Serial tangency to the caustic is in fact a consequence of Graves' theorem  \cite{miller1925}: the pair of tangents from a point $P$ on an ellipse to any confocal caustic are bisected by the ellipse normal at $P$. Equivalently, a quantity known as Joachimsthal's constant $J$ (defined below) remains invariant at every vertex of the path \cite{sergei91}.

It turns out that given a departing location, there is a dense set of initial directions for which the path switches from its normal aperiodic, space-filling regime to an N-periodic, polygonal one; see Figure~\ref{fig:definitions}(left). Through Cayley's condition \cite{dragovic88,ros2014-ellipsoids} (zeros of a determinant) yield the parameter required for a pair of conics to admit an N-periodic family, though in practice these are obtained numerically \cite{reznik2020-invariants}.

Since an N-periodic is a closed polygon interscribed between two conics, Poncelet's theorem \cite{dragovic88} guarantees a 1d family of them exists departing from any given location on the outer ellipse. Additionally, one can show that such a family conserves perimeter $L$, generally regarded as a consequence of {\em integrability}, i.e., global properties of a trajectory are fully specified by the initial conditions. Indeed, the elliptic billiard is conjectured as the only integrable planar billiard \cite{kaloshin2018,bialy2020-poritsky}. 

==> overflow.tex <==
@ARTICLE{jovanovic11-hamilton,
author={B. Jovanovi\'c},
title={What are completely integrable Hamilton systems},
journal={The Teaching  of Mathematics},
volume={13},
number={1},
pages={1--14},
year={2011},
url={http://elib.mi.sanu.ac.rs/files/journals/tm/26/tm1411.pdf}
}



